n-Step Temporal Difference Learning with Optimal n

We consider the problem of finding the optimal value of n in the n-step temporal difference (TD) learning algorithm. Our objective function for the optimization problem is the average root mean squared error (RMSE). We find the optimal n by resorting to a model-free optimization technique involving a one-simulation simultaneous perturbation stochastic approximation (SPSA) based procedure. Whereas SPSA is a zeroth-order continuous optimization procedure, we adapt it to the discrete optimization setting by using a random projection operator. We prove the asymptotic convergence of the recursion by showing that the sequence of n-updates obtained using zeroth-order stochastic gradient search converges almost surely to an internally chain transitive invariant set of an associated differential inclusion. This results in convergence of the discrete parameter sequence to the optimal n in n-step TD. Through experiments, we show that the optimal value of n is achieved with our SDPSA algorithm for arbitrary initial values. We further show using numerical evaluations that SDPSA outperforms the state-of-the-art discrete parameter stochastic optimization algorithm Optimal Computing Budget Allocation (OCBA) on benchmark RL tasks.

==> introduction_old.tex <==
\section{INTRODUCTION}
Reinforcement learning (RL) algorithms are widely used for solving problems of sequential decision-making under uncertainty. An RL agent typically makes decisions based on data that it collects through interactions with the environment in order to maximize a certain long-term reward   \cite{Bertsekas_1995,RL_Book}. Because of their model-free nature, RL algorithms have found extensive applications in various areas such as operations research, game theory, multi-agent systems, autonomous systems, communication networks and adaptive signal Processing \cite{RL_Book}. Various classes of procedures such as the action-value methods, evolutionary algorithms, and policy gradient approaches are available for finding solutions to RL problems \cite{2012_Marco}. A widely popular class of approaches are the action-value methods that solve an RL problem by learning the action-value function under a given policy, and then the learned value function is used to design a better policy. Dynamic programming, Monte Carlo (MC), and temporal-difference (TD) learning are three of the most popular action-value methods \cite{RL_Book}.  

While dynamic programming is a model-based approach, MC and TD methods are purely model-free and data-driven approaches and as a result, have been thoroughly studied in the literature. For example, the MC gradient method utilizing the sample paths is used to compute the policy gradient in \cite{Zhang2020}. Furthermore, the MC method is applied for RL-based optimal control of batch processes in \cite{Yoo2021}. Along other lines, a finite time analysis of a decentralized version of the TD(0) learning algorithm is discussed in \cite{Sun2020}. Furthermore, the TD(0) method, in combination with linear function approximation, is used for policy evaluation in \cite{Sun2021}. A variance-reduced TD method is investigated in \cite{Xu2020} that is seen to converge to a neighborhood of the fixed-point solution of TD at a linear rate. More recently, MC and TD algorithms based on function approximation using neural network architectures are being used as building blocks for deep reinforcement learning (Deep RL) \cite{Hoel2020}. In terms of adaptive algorithms, \cite{Shokri2019} presents an adaptive fuzzy approach combining eligibility traces with off-policy methods with decisions on whether or not to apply eligibility traces made during the exploratory phase. This is however significantly different from the problem that we consider. %problem and the problem setup in \cite{Shokri2019} is different from our considered problem.   

It is to be noted that, in most cases, there is no proper justification for why only regular TD, also called 1-step TD, is used and not its $n$-step  generalization for $n>1$. The $n$-step TD (for $n> 1$) tends to fall in between MC methods and 1-step TD (also called TD(0)) as MC methods are full-trajectory approaches that perform value function updates only when the entire trajectory becomes available to the decision maker. 
$n$-step TD methods have the advantage of both MC and TD requiring $n$ state transitions before beginning to perform updates. It is observed in Chapter 7 of \cite{RL_Book} that different values of $n$ in general result in different performance behaviors and so a natural question that arises is what value of $n$ to use in a given problem setting and for a given choice of the step-size parameters. However, finding the optimal value of $n$ for various problem settings is challenging and a priori an optimal $n$ for any setting cannot be found directly. We propose in this paper a two-step systematic procedure based on stochastic gradient search (though in the space of discrete parameters) that is purely data-driven and provides the optimal value of $n$ in $n$-step TD.

Methods for solving nonlinear (continuous) optimization problems include the Newton-Raphson technique, steepest descent, and quasi-Newton algorithms. %\cite{bertsekas99}. 
Most stochastic optimization algorithms are stochastic variants of their aforementioned deterministic counterparts  \cite{bhatnagar-book, Maryak2001}. 
In the case of problems where the objective function gradient is not known and only noisy objective function estimates are available (a setting previously considered by Robbins and Monro \cite{rm} in a general context), Kiefer and Wolfowitz \cite{kw} presented a stochastic optimization procedure based on finite-difference gradient approximation that requires $2$ function measurements or simulations for a scalar parameter. %When $d$ is high, such an approach would require an exorbitant amount of computation rendering it inapplicable.
In the case of vector parameters, random search procedures such as simultaneous perturbation stochastic approximation (SPSA) \cite{Spall1992}, \cite{Spallt1997} and smoothed functional algorithms \cite{bhatnagar2007} have been found to be effective as the algorithms here only require one or two system simulations regardless of the parameter dimension.  

% Gradient search procedures that are based on randomly perturbing all parameter component directions simultaneously 
% are found to be extremely useful particularly in scenarios where the parameter dimension is high. Katkovnik and Kulchitsky developed the smoothed functional technique \cite{katkul} where they approximate the objective function gradient by its smoothed version obtained by taking it's convolution w.r.t.~a Gaussian density functional. Through an integration-by-parts argument, it is then shown that the same can be rewritten as the convolution of a scaled Gaussian with the objective function itself. 
% This helps in obtaining gradient estimates that are based on exactly a single simulation regardless of the parameter dimension. Two-simulation balanced estimates such as those in \cite{stybtang, bhatnagar-book, prashanthetal} are seen to show better performance because of bias cancellation that does not happen with single-simulation algorithms. 

% In \cite{rubinstein}, a set of sufficient conditions have been provided that would make a sequence of i.i.d.~random variates candidates for smoothing density functionals. Typical candidates here are the Gaussian, Cauchy and uniform distributions respectively. In \cite{debarghya1, debarghya2}, it is observed that the $q$-Gaussian density functionals over a continuous range of $q$-values are seen to satisfy these requirements as well. 

% In \cite{Spall1992}, the simultaneous perturbation stochastic approximation (SPSA) algorithm was proposed as a noisy gradient approximation algorithm \cite{Spall1992} for finding the local minima of a nonlinear objective. Here all parameter components are simultaneously perturbed using random variates with properties that are commonly satisfied by independent symmetric Bernoulli random distribution. Because of it's ease of implementation and good performance, the SPSA algorithm is widely used in many optimization problems (e.g., statistical modeling and control). SPSA-based optimization is beneficial, especially for multivariate optimization problems in which obtaining a gradient of the objective function with respect to the parameters that need to be optimized, i.e., having an adequate system model, is difficult or impossible \cite{Spall1992}. The SPSA-based optimization procedure requires in general two system simulations for any $d$-dimensional parameter and estimates the gradient and optimizes the objective function using sample observations from these simulations. %As a result, this type of an optimization procedure is known as simulation optimization. 

% In \cite{Spallt1997}, a one-simulation SPSA algorithm is proposed where the zeroth order bias terms do not cancel away directly, however, they are seen to contribute zero in expectation. The empirical performance of this algorithm is thus not seen to be good in practice.
% As mentioned earlier, the SPSA procedure requires all parameter component directions to be randomly perturbed using symmetric independent Bernoulli distributed random variables. It has been observed in \cite{bhatnagar2003} that the performance of SPSA can be improved when the component directions are perturbed using  deterministic perturbations based on certain Hadamard matrices (HM) as these result in a regular, cyclic, cancellation of the bias terms where the cycle length is the minimum. Furthermore, with this construction, one-simulation SPSA shows better performance due to regular (cyclical) cancellation of the bias terms. 
% %SPSA-based optimization requires less simulation than other stochastic approximation (SA) based optimization techniques (e.g., finite-difference-based SA) \cite{Fu1997}.

Amongst discrete optimization methods for moderate-sized problems, ranking and selection approaches are found to be efficient \cite{bechhofer}. The optimal computing budget allocation (OCBA) is one such procedure that is based on Bayesian optimization \cite{chenlee} and is considered to be the best amongst ranking and selection procedures.
In \cite{Bhatnagar2011}, a stochastic discrete optimization problem is considered and two-simulation SPSA as well as smoothed functional algorithms that were originally devised for problems of continuous (stochastic) optimization have been adapted to the case of discrete (stochastic) optimization.  
%SPSA-based optimization can be categorized as continuous and discrete optimization. In the literature, continuous optimization is studied using random perturbation in SPSA, whereas discrete optimization is studied by using deterministic perturbation in SPSA \cite{Bhatnagar2011}.
%We mention here that one-simulation SPSA with a  deterministic perturbation sequence has not been used previously for discrete (stochastic) optimization. 
%Amongst other related work, Hadamard matrices (HM) have been found useful in other machine learning applications.
%The authors in \cite{Koutaki2018} have recently used HM for supervised discrete hashing (SDH) and found that the SDH’s training time becomes 170 times faster and the testing time, including encoding time, becomes seven times faster than the conventional SDH. Furthermore, HM is applied to online hashing in \cite{Lin2018,Lin2020}, and it is found that the proposed method outperformed various state-of-the-art methods in terms of accuracy and efficiency.
%Since the discrete optimization procedure we have is only used to update a scalar parameter ($n$), the perturbations we use are cyclic $\pm 1$-valued. In fact an HM construction would also result in the same perturbation sequence that we use. HM constructions have been found to be particularly useful in the case of algorithms involving vector-valued updates.

We present in this paper an adaptive SPSA-type algorithm except that the perturbations are deterministic, cyclic and $\pm 1$-valued. This helps us use only one simulation at any parameter update unlike SPSA that requires two simulations. 
A general treatment on deterministic perturbation SPSA is provided in \cite{bhatnagar2003}. %the simultaneous deterministic perturbation stochastic approximation (SDPSA) optimization algorithm for discrete (stochastic) optimization that we specifically use for finding the optimal value of ``$n$'' in $n$-step TD starting from an arbitrary initial value of $n$, as this falls in the realm of a discrete optimization problem. 
Our algorithm is a two-timescale stochastic approximation procedure where on the slower timescale we update the value of $n$ and on the faster scale, the {long-run average variance of the $n$-step TD estimator is obtained. In addition, the value function updates using $n$-step TD are performed that in turn feed into the long-run variance update step.} We prove the convergence of this scheme to the tuple of optimal $n$ {that minimizes the long-run variance in $n$-step TD}. We finally show the results of experiments on a setting of random walk as considered in Chapter 7 of \cite{RL_Book} where we observe that our scheme converges almost surely to the optimal value of $n$ regardless of the initial choice of the same. The contributions of our work are summarized as follows.
 \begin{enumerate}
     \item We propose a Simultaneous Deterministic Perturbation Stochastic Approximation (SDPSA) algorithm that incorporates a one-simulation discrete optimization procedure but with deterministic perturbation sequences (for improved performance) unlike regular SPSA that works on continuous settings and with  random perturbations.
     \item The proposed SDPSA algorithm is a two-timescale procedure that we employ to find the optimal value of $n$ to use in $n$-step TD, starting from any arbitrary initial value of the same that we show results in regular bias cancellation from the use of deterministic perturbations. 
     %\item SDPSA is useful in finding the pair of the optimal $n$ and its corresponding value function to which it converges in a given setting, as the same $n$ is not expected to work in every setting.
     \item We prove the convergence of SDPSA and show that it finds the optimal $n$ {that minimizes the long-run variance in $n$-step TD}. 
     \item Our experimental results show that the optimal value of $n$ is achieved with SDPSA for any arbitrary initial value of the same.\footnote{{The code for our experiments is available on \url{https://github.com/LakshmiMandal/n_stepTD_opt_n}}}
     \item To the best of our knowledge, ours is the first work to propose a systematic procedure for finding the optimal value of $n$ in $n$-step TD. 
 \end{enumerate}

%The rest of the paper is organized as follows. \Cref{methodology} describes our proposed methodology. Convergence analysis of the proposed algorithm is described in \Cref{conv_analysis}. \Cref{exp_results} presents the results of experiments of our algorithms. \Cref{conclusion} provides the conclusions and gives pointers to further research.

% Our focus in this paper specifically is on the $n$-step TD method and our objective is to find the optimal value of $n$ when using $n$-step TD. Obviously the optimal value of $n$ for different problem settings would in general be different and our procedure constitutes a model-free method for finding the optimal $n$ only when sample realizations are made available.

% In the literature, SPSA-based optimization techniques are mainly studied for continuous optimization with random perturbations \cite{Spall1992}. However, the SPSA procedure can be adapted for discrete parameter optimization in conjunction with deterministic perturbation sequences. The Hadamard Matrix (HM) can be used to generate deterministic perturbation sequences. HM is named after Jacques Hadamard, a French mathematician. It's a square matrix. This matrix's entries are either +1 or -1, and its rows are mutually orthogonal. James Joseph Sylvester constructed Hadamard matrices for the first time in 1867. Recently, the HM is used for supervised discrete hashing (SDH) \cite{Koutaki2018}. The authors demonstrated that their proposed SDH's training time is 170 times faster and testing time, including encoding time, is seven times faster than conventional SDH. Furthermore, the HM is applied to online hashing \cite{Lin2018,Lin2020}. The authors demonstrated that their proposed method outperformed various state-of-the-art methods in terms of accuracy and efficiency. However, the Hadamard matrix-guided SPSA-based optimization algorithm (DP-SPSA) employs deterministic perturbation to find the optimal value of ``$n$'' in $n$-step TD starting from an arbitrary value of $n$, which has never been reported in the literature.
 

% In this paper, we have used a model-free optimization technique, such as simultaneous perturbation stochastic approximation (SPSA), to find the optimal value of $n$ from an arbitrary $n$. 

% Temporal difference (TD) learning is a popular and widely used RL algorithm \cite{Sutton_1988} for the problem of prediction. Like MC, TD gains experience through sampling but unlike the former that is a trajectory-based method, it incorporates bootstrapping. It's value updates of any state are based on the value updates of other states and so  It reduces the variance of evaluations while increasing bias, but it usually improves learning performance. The term temporal differences refers to how the previous estimate of the state value in the following time step influences the current estimate of the state value in the current time step. TD method can take time steps one, two, three until termination (this is MC method). That is MC and TD methods can be unified as $n$-step TD method and optimal $n$-step TD method can be used for a specific tasks. However, in the literature, the Monte Carlo (MC) method and TD(0) method as TD method are rigorously studied \cite{RL_Book}. 

% Among TD methods, TD(0) algorithm is the most dominant and celebrated one. This algorithm appears frequently in the literature \cite{RL_Book}.
% It employs the Bellman equation to iteratively bootstrap the estimation process and incrementally update the value function.
% $n$-step algorithm provides a bridge from TD to Monte Carlo method.

% In our work, the one-step temporal difference (TD) \cite{RL_Book} and the Monte Carlo (MC) \cite{Vodopivec2017} methods are unified. Neither the MC nor the one-step TD method is always best. These are two extremes. It is often observed that intermediate of these two extremes is best to serve a specific task. Thus, a generalized $n$-step TD method can be considered to perform a particular task. One of the advantages of a $n$-step TD method is that this method has freedom to choose the time step. On the other side, One-step TD method does not have this freedom. In this method, the same time step determines how often the action can be changed and bootstrapping can be done. In many applications, it is desirable to update the action very quickly so that changes reflect then and there. We know that, bootstrapping works best when it is done over a period of time, where a significant state change occurred. Thus, a compromise must be made because of the same time intervals in one-step TD methods. On the other hand, bootstrapping can take place over multiple steps in $n$-step methods. The concept of $n$-step method is primarily used to introduce the algorithmic concept of eligibility traces. This concept allows bootstrapping over multiple time intervals at the same time. In this work, we consider the $n$-step bootstrapping concept, separated from the  eligibility traces.
% Consider estimating value $v_{\pi}$ from sample episodes generated using policy $\pi$. MC method performs an update for each state based on the entire sequence of observed rewards from that 
% state (that is the current state) until the end of the episode. The update of one-step TD method, on the other hand, is based on the just the one next reward. One-step method uses the value of the state which is one step later the current state. The value of the next state works as a proxy for the remaining rewards. One kind of intermediate method is update of the current state value based on an intermediate number of rewards. This number is more than one, but less than all of rewards until termination. Thus, in the $n$ step TD method $n$ can take values two, three, four and so on. For example, a two-step TD method is based on the first two rewards and the estimated value of the state two steps later. In the similar manner, update of a three-step TD method, a four-step TD method is done. Thus, the question is, for a specific task, what is the optimal value of $n$ in $n$-step TD method and how can we get it.

%Write literature servey of SPSA
% Our objective in this paper is to determine the optimal value of $n$ (i.e., $n^*$) within a discrete set of parameters that minimizes the error (i.e., cost function) of the $n$-step TD algorithm. In this case, simulating trajectories can be used to estimate the long-run average cost. For our problem, we can consider simulation optimization. 
 % Techniques for simulation optimization have been investigated for both continuous and discrete valued parameters. The problem addressed in this paper falls under the category of discrete parameter simulation optimization. The simultaneous perturbation stochastic approximation (SPSA) algorithm is really very effective for multivariate optimization problems where obtaining a gradient of the objective function with respect to the parameters being optimised is challenging or impossible \cite{Spall1992}. In \cite{Fu1997}, authors discussed Optimization of discrete event systems using simultaneous perturbation stochastic approximation. Furthermore, SPSA algorithm is extensively  studied in \cite{Bhatnagar2011,Maryak2001,He2003}. However, in the literature, SPSA technique is not applied to find the optimal "n" in $n$-step temporal difference. 

==> methodology_old.tex <==
\section{THE PROPOSED METHODOLOGY}
\label{methodology}

This section describes our proposed SDPSA algorithm (\Cref{SPSA}) for determining the optimal $n$ for the $n$-step TD (TD($n$)) algorithm (\Cref{n_step_TD}) (see \Cref{fig:flowchart_converged_RMSE_diff_n} (a)).
% A modular structure of the proposed SDPSA algorithm is created, which is presented in \Cref{fig:flowchart}, to facilitate better understanding of how the algorithm works and is implemented. For better understanding, firstly TD($n$) algorithm (see \Cref{n_step_TD}) is explained and then the proposed SDPSA algorithm (see \Cref{SPSA}) is presented. The TD($n$) algorithm, for a given value of $n$, is seen to converge to the solution of the $n$-step Bellman equation for a given policy.

% \begin{figure}
%     \centering
%     \includegraphics[width=1.5in]{images/SDPSA_n_Step_TD_Flowchart.pdf}
%     \caption{Flowchart of the proposed algorithm.}
%     \label{fig:flowchart}
%     \vspace{-14pt}
% \end{figure}

\subsection{$n$-step TD (TD($n$)) Algorithm}

\begin{algorithm}[htb]
%	\vspace{-10pt}
\caption{TD($n$) Algorithm}
\label{n_step_TD}

{\textbf{Input:} a policy $\pi$, $n$, $\alpha$, initial arbitrarily $V_n(s)$ $\forall s \in S$, $J(n)=0$}.

% \textbf{Parameters:} $n$, $\alpha$.

% \textbf{Initialize:} $V_n(s)$ arbitrarily, $\forall s \in S, J(n)=0$.

{\textbf{Output:} Converged value of $V_n(s)$ $ \forall s \in S$ and $J(n)$.}

\For {$e$ in episodes:}{

    Initialize: $S_0$ and set as non-terminal state
    
    Termination time, $T \leftarrow \infty$

    \For {$i=0,1,2,\dots$}{

        \If {$i < T :$}{

            Action $\sim \pi(\cdot \mid S_i)$ 
            
            {Observe reward $R_{i+1}$, next state $S_{i+1}$} 

            \If {$S_{i+1}$ is terminal state:}{

                $T \leftarrow i+1$}}

        $\kappa \leftarrow i-n+1$

        \If {$\kappa \geq 0:$}{

            ${\hat V_n}(S_\kappa)\leftarrow \sum_{j=\kappa+1}^{\min (\kappa +n ,T)} \gamma^{j-\kappa-1}R_j $

            \If {$\kappa +n < T:$}{

                ${\hat V_n}(S_\kappa) \leftarrow {\hat V_n}(S_\kappa) + \gamma^n V_n(S_{\kappa + n})$}

            $V_n(S_{\kappa}) \leftarrow V_n(S_{\kappa})+ \alpha[{\hat V_n}(S_\kappa)-V_n(S_{\kappa})]$

            {$g_n(S_{\kappa})\leftarrow (\hat V_n(S_{\kappa})-V_n(S_{\kappa}))^2$}
            
            $J(n) \leftarrow J(n) + \alpha[g_n(S_\kappa) - J(n)]$
            }}

        Until $\kappa = T-1$}
\end{algorithm} 

% As explained previously, we provide here an algorithm that adaptively finds the optimal value of $n$ to use for the TD($n$) algorithm. The same `optimal' $n$ is not expected to work in every setting and so our algorithm is useful in finding the pair of the optimal $n$ and the corresponding value function to which it converges for the given setting.

Our proposed algorithm is a two-time scale stochastic approximation scheme wherein the TD($n$) algorithm runs along the faster timescale for any prescribed value of $n$ that in-turn gets updated on the slower timescale along the gradient descent direction. The basic underlying setting is of a Markov decision process (MDP), which is defined via  the tuple $<S; A; P; R; \gamma>$, where $S$, $A$, $P$, $R$, and $\gamma \in (0,1]$ represent the state space, the action space, the transition probability function, the reward function, and discount factor, respectively. The state and action spaces are assumed here to be finite.

We now describe the TD($n$) algorithm (see \Cref{n_step_TD}). %Recall that the TD($n$) algorithm deals with the problem of prediction, i.e., it estimates the value function of a given policy. 
Here, a policy $\pi$, which maps the state space $S$ to the action space $A$, is input to the algorithm. The {input} parameters of \Cref{n_step_TD} are a positive integer $n$ and a step-size $\alpha \in (0,1]$. %The quantity $n$ defines the number of steps in TD($n$) to wait after which an update to the value of the state at the given instant is performed. 
The value function {$V_n(\cdot)$, for a given $n$}, for each state $s \in S$ is initialized arbitrarily. {Here $R_t\stackrel{\triangle}{=} R(S_{t-1},\pi(S_{t-1}), S_t)$ is the reward obtained at instant $t$}. The state–reward sequence obtained under $\pi$ is then denoted as $S_0$, $R_{1}$, $S_{1}$, $R_{2}$, $S_2$, $\dots$, $R_T$, $S_T$, where $T$ is the termination time of the episode. Note that the procedure here works in the case of both stochastic shortest path (i.e., episodic) problems as well as infinite horizon discounted reward problems. In the latter case, $T$ can denote some a priori chosen termination time for each episode. %as infinitely long trajectories cannot be generated in practice and moreover, because of the discount factor, trajectories that are very large in length would not be required for the procedure.
\begin{figure}[b]
\centering
\vspace{-60pt}
  \subfloat[]{
	\begin{minipage}[c][1\width]{
	   0.5\textwidth}
	   \centering
        \includegraphics[width=0.86\textwidth]{images/SDPSA_n_Step_TD_Flowchart.pdf}
        \vspace{-60pt}
	\end{minipage}}	
  \subfloat[]{
	\begin{minipage}[c][1\width]{
	   0.5\textwidth}
        \hspace{-30pt}
	   \centering
	   \includegraphics[width=0.86\textwidth]{images/converged_RMSE_diff_n/converged_RMSE_diff_n.pdf}
    \vspace{-60pt}
	\end{minipage}}
 % \vspace{-10pt}
\caption{{(a) Flowchart of the proposed algorithm. (b) RMSE values w.r.t. different values of $n$ and fixed $\alpha$.}}
\label{fig:flowchart_converged_RMSE_diff_n}
\vspace{-10pt}
\end{figure}
%We use $S_0$ to denote the initial state and $i$ the time instant. Further, $\kappa$ is the time instant whose state's estimate is being updated. 
The $n$-step return of TD($n$) for the state visited at instant $\kappa$ in the trajectory is denoted by ${\hat V_n}(S_\kappa)$, where for $\kappa=i$,
\vspace{-5pt}
\begin{equation}
\label{hatV}
\vspace{-5pt}
{\hat V_n}(S_i) \doteq \sum_{j=1}^n \gamma ^{j-1}R_{i+j} +\gamma^n V_n(S_{i+n}),
\end{equation}
$\forall n\geq 1$ and $0 \leq i< T-n$. In this algorithm, ${\hat V_n}(S_i)$ is the $n$-step return used in TD($n$) counted from instant $i$ when the state is $S_i$. The quantity $V_{n}(S_{i+n})$ denotes the estimate of the value of state $S_{i+n}$ %that is available at instant $i+n-1$ 
provided the given trajectory hasn't terminated until instant $i+n$. 
If, on the other hand, the trajectory terminates before $i+n$, the return ${\hat V_n}(S_i)$ becomes the Monte-Carlo return, cf.~Chapter 7 of \cite{RL_Book}. Further, {the error term $g_n(\cdot)$ and its long-term average $J(n)$ or long-run mean-squared error (MSE)} are explained in the subsequent section.
{To show the effect of $n$ and $\alpha$ on $J(\cdot)$, additional numerical simulations on the example of Random Walk studied in \Cref{exp_results} and using \Cref{n_step_TD}, are displayed in  \Cref{fig:flowchart_converged_RMSE_diff_n}(b) which shows plots of the square-root of $J(n)$, i.e., RMSE, obtained upon convergence of Algorithm 1 for each value of $n$. It is evident that the RMSE and hence $J(n)$ does not increase with n.} 
% the outcome of additional numerical simulations considering the example of Random Walk as in \Cref{exp_results} and using \Cref{n_step_TD}, shows how the square-root of converged $J(n)$, i.e., root-mean-squared-error (RMSE), varies with $n$ for given $n$ and a fixed $\alpha$ and the variation of the converged RMSE with $\alpha$. 
% In particular \Cref{fig:flowchart_converged_RMSE_diff_n}(b) 

%since the reward from then on as well as all the value estimates of the state when termination has happened are identically zero. Note that TD($n$) falls mid-way between Monte-Carlo and one-step TD. 

%The TD-error $(C_\kappa(n)-V(S_\kappa))^2$ accumulated from \Cref{n_step_TD} is used as an estimated cost in \Cref{SPSA}, that runs on the slower timescale and  updates the value of $n$.

% \subsection{Calculate-RMS Algorithm}

% \begin{algorithm}[t]
% \caption{Calculate-RMS Algorithm}
% \label{RMS}

% \textbf{Input:} number of episodes as $NE$.

% number of states as $NS$.

% \For {e in episodes:}{

%     $\rho$=0

%      Execute \Cref{n_step_TD} and receive $\hat V$

%     $\rho \leftarrow \rho+ \sqrt(\frac{1}{NS}\sum_{s=1}^{NS}{(V(s) - \hat V(s))}^ 2)$ } 
% Return $J(n)= \rho / NE$  
% \end{algorithm}

% In Calculate-RMS algorithm (i.e., \Cref{RMS}), the total number of episodes $NE$ and the total number of states $NS$ to use in the TD($n$) algorithm are taken as input. For each episode, the TD($n$) algorithm is executed to get an estimated state-value, which is utilized to calculate the RMS error (simply referred to as RMS). In \Cref{RMS}, $ \rho, V(s)$, and $\hat V(s)$ denote the RMS, the actual value of state $s$, and the estimated value of state $s$, respectively. At the end of the last episode, the average episodic RMS error $J(n)$ is calculated and returned to the proposed SDPSA algorithm.

\subsection{The Proposed SDPSA Algorithm}
% \vspace{-10pt}

%For improved clarity, the framework of the proposed SDPSA algorithm is discussed first and then the algorithm is explained. 
For our algorithm, we consider a deterministic sequence of perturbations whereby the perturbation variable $\Delta$ used to perturb the parameter is set equal to $+1$ on every even iteration ($k=0,2,4,\ldots$) and to $-1$ on every odd iteration ($k=1,3,5,\ldots$). 
%Thus, the proposed algorithm is named SDPSA %(where DP stands for deterministic perturbation).
Note that the underlying process is a discrete Markov process $\{S_{m}\}$, i.e., the state-valued sequence that does not depend on the parameter $n$. {The latter only impacts the value estimation procedure and not the state evolution}. Now, $n \in D \subset \mathcal{Z}^+$, a finite set of positive integers. %Let $D=\{d^0,\dots,d^N\}$, with $d^0<d^1< \dots <d^N$, where, $D_{min} := d^0$ and $D_{max}:= d^{N}$. Now, let $D$ is known and contains $l$ points 
Thus, let $D=\{1,2,\dots,L\}$ for some $L$ large enough and let $\bar D$ denote the closed convex hull of $D$, viz., $\bar D=[1, L]$. The SDPSA algorithm updates the parameter $n$ within the set $\bar D$. For $x\in \bar{D}$, $\Gamma(x) \in D$ is the projection of $x$ to $D$.

% The considered notations and assumptions of the SDPSA algorithm are as given below.

% % {\textbf{Notations and Assumptions:}}
% \begin{itemize}
%     % \item $\mathcal{Z}$: Set of integers.
%     \item $\mathcal{Z}^+$: Set of all positive integers.
%     \item $D$: A finite subset of $\mathcal{Z}^+$.
%     \item Let $D=\{d^0,\dots,d^N\}$, with $d^0<d^1< \dots <d^N$.
%     \item Let, $D_{min} := d^0$ and $D_{max}:= d^{N}$.
%     \item Set $D$ is known and contains $l$ points.
%     \item Thus, $D=\{n^1,n^2,\dots,n^l\}$.
%     \item In this work, $X_m^n$, $m\geq 0$ takes values in the state space $S=\{0,1,\dots,\mid S \mid\}$, $\mid S \mid<\infty$.
%     \item Let, $\bar D$ denote the closed convex hull of $D$ and $\bar D=[D_{min}, D_{max}]$.
%     \item The SDPSA algorithm performs update of parameter ``$n$'' within the set $\bar D$. 
%     \item For $x\in \bar{D}$, $\Gamma(x) \in D$ is the projection of $x$ to $D$.
% \end{itemize}

We assume that the state-process $\{S_m\}$ is ergodic Markov and takes values in the state space $S=\{0,1,\dots,|S|\}$, $|S|<\infty$. We denote the transition probability from state $x$ to state $y$ for the process $\{S_m\}$ to be $p_{xy}$, $x,y \in S$. Let $g_n(S_i)\dot{=}({\hat V_n}(S_i)-V_n(S_i))^2$ be the single-stage cost when the parameter value is $n$ and the state is $S_i$ at instant $i$. Thus, we consider the {long-run mean-squared error $J(\cdot)$ or the long-run variance of $\hat V_n$,} as the objective function to minimize. %i.e., an $n$-step TD update is run, see Algorithm \ref{n_step_TD}, whose long-run average we denote by $J(\cdot)$. 
A desired global minimizer (i.e., $n^* \in D$) of $J(\cdot)$ will satisfy 
\vspace{-5pt}
\begin{equation}
\vspace{-5pt}
\label{eq:costFun}
    J(n^*)= \lim_{m \rightarrow \infty} \frac{1}{m}\mathbb{E} \left[\sum_{i=1}^m g_{n^*}(S_i)\right]=\min_{n \in D} J(n).
\end{equation}
The limit in (\ref{eq:costFun}) exists since $\{S_m\}$ is ergodic ({that also ensures the existence of a unique stationary distribution for the Markov chain under the given policy}) regardless of $n\in D$. 
Moreover, two projections $\bar \Gamma$ and $\Gamma$ are considered to respectively update the parameter in the set $[1,L]$ and determine the actual parameter to be used in the simulation. For the latter, we use a method of random projections to arrive at the parameter value to use from within $D$ given the update in $\bar{D}$ as follows: For $k\leq n \leq k+1$, $1\leq k<L$,
\vspace{-5pt}
\begin{equation}
\vspace{-5pt}
    \label{eq:projection}
    \Gamma(n)=
    \begin{cases}
      k, &  \text{w.p.} \ (k+1-n) \\
      k+1, & \text{w.p.} \ (n-k)
    \end{cases}
  \end{equation}
and for $n<1$ or $n>L$, we let
\vspace{-5pt}
\begin{equation}
\vspace{-5pt}
\label{eq:projection_bound}
    \Gamma(n)=
    \begin{cases}
      1, &  \text{if} \  n< 1\\
      L, & \text{if} \ n \geq L
    \end{cases}
  \end{equation}

%The w.p. symbol in (\ref{eq:projection}) stands for with probability. 
In (\ref{eq:projection}), we use the fact that $n=\beta k+(1-\beta)(k+1)$, $k \leq n \leq (k+1)$, for some $\beta\in [0,1]$, with $k,k+1\in D$. Thus, $\beta=(k+1-n)$ and $1-\beta = (n-k)$, respectively. The lower and upper bounds of the projected values of $n$ are $1$ and $L$, respectively, and are taken care of by (\ref{eq:projection_bound}). $\bar\Gamma$, on the other hand, is the operator that projects any point $n \in \mathbb{R}$ to the set $\bar{D}$ (the closed and convex hull of $D$) and is simply defined as $\bar\Gamma(n)=\min(L,\max(n,1))$. {From the foregoing, a natural way to define the value function estimate $ \hat V_n$ for $n\in \bar{D}$ and in particular, $k\leq n\leq k+1$, would be as follows:
\[
\hat{V}_n(x) = \beta \hat{V}_k(x) + (1-\beta)\hat{V}_{k+1}(x),
\]
where $\hat{V}_k$ and $\hat{V}_{k+1}$ respectively correspond to $\hat{V}_n$ in (\ref{hatV}) but with $n$ replaced by $k$ and $k+1$. }
Two step-size sequences, $\{a_m, m \geq 0\}$ and $\{b_m, m \geq 0\}$ {are employed that satisfy the following conditions:} %Together with the sequence $\{\delta_m,m\geq 0\}$, these satisfy the following: 
$a_m,b_m >0$, $\forall m\geq 0$. Further, 
\vspace{-7pt}
\begin{equation}
\vspace{-5pt}
\label{stepSize1}
 \sum_{m} a_m=\sum_{m} b_m= \infty;
 \mbox{ } \frac{a(k+1)}{a(k)}
 \rightarrow 1 \mbox{ as } k\rightarrow \infty; 
 \end{equation}
% \vspace{-3pt}
\begin{equation}
\vspace{-3pt}
\label{stepSize2}
 {\sum_m a_m^2 <\infty}; \sum_m b_m^2 <\infty; \mbox{ } {\lim_{m\rightarrow \infty} \frac{a_m}{b_m}=0}.
\end{equation}
\vspace{-5pt}

The conditions in (\ref{stepSize1}) are needed for proving the convergence of the scheme. The first two conditions in \eqref{stepSize2} ensure convergence of the martingale sequences associated with the recursions. Also, the last condition in (\ref{stepSize2}) ensures that $a_m$ tends to zero at a rate faster than $b_m$ and thus the (slower) approximate gradient recursion governed by $a_m$ can be treated to be quasi-static from the view-point of the timescale of $\{b_m\}$ while from that of $\{a_m\}$, the recursion governed by $\{b_m\}$ would appear to be equilibrated. %The conditions in \eqref{stepSize3} are required in the proof of Theorem~\ref{theorem1}. %These conditions are seen to be easily satisfied by step-sizes of the form $k_0/m^\gamma$ for suitable choice of $\gamma$ for $a(m),b(m)$ as well as $\delta_m$.

In our work, $b_m$ is used to estimate both the value function as well as the average cost using a single simulation with a perturbed parameter, whereas $a_m$ is employed to update the parameter in the SDPSA algorithm. For our implementations, however, we used constant step-sizes  $\nu$ and $\alpha$ (see \Cref{SPSA} and \Cref{n_step_TD}) with $\nu < \alpha$, in place of $a_m$ and $b_m$ as our aim there is to demonstrate the effectiveness of the proposed algorithm on the experiment in Chapter 7 of \cite{RL_Book} where the step-size $\alpha$ is held fixed. %As mentioned before, the TD($n$) recursion runs on a faster timescale, while the SDPSA procedure us run on a slower timescale. 

\begin{algorithm}[t]
\caption{The SDPSA Algorithm}
\label{SPSA}
{\textbf{Input:} Initial value of $n=n_0$, parameters $\nu$, $\delta$, $\Delta$.}

% \textbf{Parameters:} step-size $\nu$, $\delta$, $\Delta$.

 {\textbf{Output:} Optimal value of $n=n^*$.}
 
$\Delta = +1$ for $k= 0,2,4,6,8,\ldots$

           $= -1$ for $k= 1,3,5,7,\ldots$
           
\For {$k=0,1,2\dots$}{

    $ {n:=}\min(L,\max(1,\Gamma(n + \delta \Delta)))$

    {Call \Cref{n_step_TD} to get $J(n)$, $\hat{\dot J}(n) :=\frac{J(n)}{\delta \Delta}$.}

    $n \leftarrow n- \nu * {{\hat{\dot J}}}(n)$ ({use (\ref{eq:re_n_update_rule}) $-$ (\ref{TD_state_value_update})} )}

Return optimal $n$
% \end{algorithmic}
\end{algorithm}
In the proposed SDPSA algorithm (see \Cref{SPSA}), $n$ is initialized to some $n_0\in D$. %The parameters of \Cref{SPSA} are the step-size $\nu$, $\Delta$ and a given $\delta_m\equiv \delta$. 
The SDPSA, unlike regular SPSA, utilizes a deterministic perturbed sequence (i.e., $ \{\Delta_m\}$) with $\Delta_m=+1$ (resp.~$-1$) for $m$ even (resp.~odd). This choice for the perturbation sequence ensures that the bias terms in the gradient estimates cancel cyclically and so the bias in the algorithm does not grow as the recursions progress. %An advantage with our algorithm unlike the algorithms (that use two function measurements) in \cite{Bhatnagar2011} is that it is a one-measurement (or one-simulation) procedure that estimates the gradient of the RMS error. 
%The update rule is the following (here $n_m$ is the value of $n$ at iterate $m$ in the procedure):
%\vspace{-5pt}
%\begin{equation}
%\vspace{-5pt}
%\label{eq:n_update_rule}n_{m+1}= %\bar{\Gamma}\left(n_{m}-a_m \frac{J( %\Gamma(n_m+\delta_m \Delta_m))}{\delta_m %\Delta_m}\right).
%\end{equation}
 The projected parameter $\Gamma(n_m+ \delta \Delta_m)$ is calculated and used for the value function estimate and that in turn gives the error term for the TD($n$) update. %The value of $n$ is updated using (\ref{eq:n_update_rule}). 
% Upon convergence of the SDPSA algorithm, the optimal value $n^*$ is obtained. %We now elaborate the aforementioned procedure by also presenting how one estimates $J(\Gamma(n_m+\delta_m \Delta_m))$. %As mentioned earlier, the
%actual procedure we implement incorporates two timescale schedules. 
Let $n_m$ denote the value of $n$ in the $m$th update of the recursion, $Y_m$ be the running estimate of the long-run average cost and $V_m(i)$ the $m$th update of the value of state $i$.
The following is the set of updates:
%Two-timescale recursions (\ref{eq:re_n_update_rule}) and (\ref{eq:re_grad_J}) are used here.
\vspace{-5pt}
\begin{eqnarray}
\label{eq:re_n_update_rule}
n_{m+1}&=& \bar{\Gamma}\left(n_{m}-a_m \frac{Y_{m+1}}{\delta \Delta_m}\right),\\
%\vspace{-5pt}
\label{eq:re_grad_J}
    Y_{m+1}&=&Y_m+b_m \left( {g_{n_m}}(S_m) - Y_m \right),\\
\label{TD_state_value_update}
V_{m+1}(i) &=& V_m(i) + b_mI_{S_m}(i)({\hat V_{n_{m}}}(i) - V_m(i)), 
\end{eqnarray}
$i\in S$. 
Here $I_{S_m}(i) =+1$ if $S_m=i$ and $0$ otherwise, denotes the indicator function.
%The state-value in TD($n$) is updated using (\ref{TD_state_value_update}) below.% as future rewards are not available for use in the algorithm.

%where, $ 0 \leq i<T,$ and, $V_{i+n}(s) = V_{i+n-1}(s), \forall s \neq S_i$.
%Thus, SDPSA is a two-time scale one-measurement data-driven discrete optimization algorithm. 
%In the next section, the convergence of this algorithm is analyzed.
